Man-in-The-Middle Attacks and Defense in a Power System Cyber-Physical Testbed

Man-in-The-Middle (MiTM) attacks present numerous threats to a smart grid. In a MiTM attack, an intruder embeds itself within a conversation between two devices to either eavesdrop or impersonate one of the devices, making it appear to be a normal exchange of information. Thus, the intruder can perform false data injection (FDI) and false command injection (FCI) attacks that can compromise power system operations, such as state estimation, economic dispatch, and automatic generation control (AGC). Very few researchers have focused on MiTM methods that are difficult to detect within a smart grid. To address this, we are designing and implementing multi-stage MiTM intrusions in an emulation-based cyber-physical power system testbed against a large-scale synthetic grid model to demonstrate how such attacks can cause physical contingencies such as misguided operation and false measurements. MiTM intrusions create FCI, FDI, and replay attacks in this synthetic power grid. This work enables stakeholders to defend against these stealthy attacks, and we present detection mechanisms that are developed using multiple alerts from intrusion detection systems and network monitoring tools. Our contribution will enable other smart grid security researchers and industry to develop further detection mechanisms for inconspicuous MiTM attacks.

==> Content/6_future_work.tex <==

\section{Future Work}
\label{future_works}






==> Content/feedbacks.tex <==
\section{Feedbacks}
\begin{enumerate}
    \item {\textbf{Review 1:} This paper provides the design of a testbed for energy systems, and provides a use case consisting of two simple attacks (DoS and MITM) on the testbed, measuring the effect. Whilst the design of a testbed is a valuable endeavour, it is currently not clear as to the use cases the testbed aims to support. In general, the design is not clearly motivated beyond the need for data on attacks. But the two presented attacks are detectable by existing IDS mechanisms so what is the purpose of the dataset collection? If the novelty lies in the design of the testbed then limitations of existing (related) testbeds need to be clearly articulated and also what are the use cases that won't be supported as a result of those design limitations that the new testbed addresses. The abstract, introduction and related work are very much focused on the build of a testbed with the attacks bing simple use cases, however most of the remainder of the text in the paper is on testing the two attacks. The testbed design section needs further detail on the design and operation of the individual components, with clearer, and larger, architecture diagrams. This also needs to be backed by motivation and background on real-world energy systems to show why this testbed architecture provides a realistic environment for evaluation. The paper refers to two Github repositories where code for the system is hosted to cover some details missing from the paper, however these repositories are restricted access. The two attacks, DoS and MiTM, are fairly generic and do not provide novelty. It would perhaps be better to provide more tailored attack examples for the energy sector, and in evaluating them explore the impact on the underlying process. We know that a DoS attack will slow down the network, but what does that mean for DNP3 in the energy environment? Finally, the paper implements very simple detection using snort rules, however these are not new rules and do not provide much novelty, despite "detection" being included in the paper title.
    
    Section Specific Comments:  Related work - It would be good to see a little more on attacks against DNP3 here, including specific devices. Are there any MiTM/DOS CVEs for devices in the power systems space? Final paragraph should probably be moved to Section 3. Some background on a typical architecture for a power system would help frame the paper better for a less familiar reader, and provide a motivation for the design of the testbed, as well as a point of reference for how well the testbed matches a real-world system. Section 3 - Architecture: Figures 1 and 2 are quite unclear, both due to low resolution and layout. 3.1 The text references the red attacker subnet in Figure 2, however there are only 2 subnets shown in the figure in blue and green. 3.2 The code reference (26) is behind a Tamu login screen and so inaccessible 3.4 It is unclear is CyPRES is a new application, or an existing application. CyPRES is not mentioned explicitly in Figures 1 or 2, though I assume it is the "central -application". 3.5 The referenced repo (reference 27) is also behind a Tamu password. What sort of attacks is snort configured to detect? There is no coverage of the RTAC accelerator in this section.  Section 4 - Threat model- 4.1 The threat model includes specifics on how the attacks will work, but misses the higher level of the attacker type and what their goal is. What is the goal of the attacker? To shut down the power system? The Stuxnet and Ukraine attacks descriptions would be better placed in a background section within the related work. 4.2 The term "Ping-of-death" is used, however a ICMP flood is a more accurate description of the attack described. Table 1 and Algorithm 1 - This table and algorithm do not add much information on top of the text. These could be removed to allow for more space to enlarge the system diagrams to make them clearer. 4.2 Attack description is good, however the MiTM attack only operates in one direction. This means that when the command is switched from trip to close, the response from the outstation shows the closed state, which would be a big indicator for the DNP3 master. This is clearly shown in Fig 5. Why does the attack not modify this response so the DNP3 master has an incorrect view and thinks it's correct command was carried out? Section 5 -- 5.2 Fig 6 and 7 is a bit unclear on how the increasing payload size and interval time has an impact. There are no axis labels or data points labels which show what the payload size or interval are. 5.2.1 The same comment (as above) applies to figures 8 and 9. Labels to indicate when individual attacks start and stop would make the diagram a lot easier to understand, or move to a diagram where all attacks of different sizes are plotted as individual lines to allow a better comparison 5.3 The exploration of the MiTM attack is very limited when compared to the DoS attack. Some insight of the effect of this attack on the power grid would be very nice here. 5.3.1 Is RTT increase really a big issue with the MITM attack, when the attack can have a potentially catastrophic impact on the process below. An attacker could see the RTT has increased, but they could also simply see that the response mismatches the request (see comment on 4.2). And the attack is modifying the packet in transit, so the sequence number should stay the same. 5.4 This snort rule is purely looking for ICP packets rather than a flood, and so would throw a lot of false positives.
}

\item{\textbf{Review 2:} This paper builds upon previous work by the authors for developing a power grid testbed. While in their earlier work, they focused on the physical aspects of the power grid, in this paper, they concentrate on building the communication network. Overall this appears to be the main contribution of this paper: the integration of previous physical models of the grid with a computer network and then showing that the network can be used to launch and detect basic attacks. From a security perspective, this paper offers very little; it appears to be more a paper for a power grid or simulation conference or workshop. Still, on the other hand, I admire the efforts of the authors for putting this system together. It is engineering work, so there is little research contribution here, but it is nonetheless a lot of work and, therefore, a reasonable contribution to this workshop. It would be useful to give a brief overview of SCADA protocols and why they chose DNP3 to evaluate their framework.

A description of the DNP3 protocol is missing. For example, a description of the DNP3's packets' structure would be suitable for a better understanding of the Packet processing in the MiTM attack. Compared to other works, explain in more detail what makes this testbed different from others. Description and explanation of the purpose of using physical SEL relay and RTAC units. Improve the quality resolution of figures 1 to 4.}


\item {\textbf{Review 3:}This paper outlines the development of two well-known attacks against a power system testbed emulating realistic components in a power grid network. A DoS attack was launched (assuming that an attacker already gained control of an internal node) by using a "Ping of Death" style attack where the attacker-controlled system sends out a flood of ICMP echo packets. This particular attack was shown to drastically affect the average roundtrip time (RTT) of packets sent in the network, as expected. The authors demonstrate that a single line rule can be added to the Snort IDS configuration file to detect this attack. Further, the authors developed a slightly more complex man-in-the-middle attack (which again assumes that an attacker was able to compromise an internal node). This attack first employs ARP spoofing to impersonate the DNP3 outstation and then serves as an intermediary between the actual outstation and the substation network. Now, the attacker is able to view data going both ways and can inject false data to influence the operation of the devices in the power system in malicious ways. The authors demonstrated that this attack could also be readily detected by Snort by introducing a few rules to the configuration file. Overall, this work reiterates two existing and well-studied attacks that are shown to be easily detected by modern intrusion detection systems. Also, these same attacks have been launched against existing cyber physical test beds and power systems such as [4, so it is unclear what sets this work apart from previous efforts. More complex attacks that are not easily detected by existing countermeasures and highlight shortcomings of these current defenses would be more beneficial to the cybersecurity community. Nevertheless, this paper in its current state is not clearly motivated, given that related works already offer a list of existing testbeds. The authors should elaborate what are the new features their testbed provides; the latter is paramount to determining the impact of this paper and should not be left for future work.  Another way to improve this manuscript is to add and fix several occurrences of punctuation mistakes, such as several missing periods (this is most noticeable in Section V). Lastly, the text in most figures is hard to read and should be made larger to add more value to the paper and complement the text more.}

\item{\textbf{Review 4:} To evaluate different cyber attacks impact to power system, in this paper the authors built a power system testbed using several components such as PowerWorld Dynamic Studio (DS) and Common Open Research Emulator (CORE). Then they utilized the testbed to test Denial of Service (DoS) attack and Man-in-the-Middle (MitM) attack.

Strengths : A testbed consists of many well-known component. A comprehensive experiment to collect many aspects of data.

Weaknesses: No new discovery is provided and the used analysis approach is well discussed.
The experiment data, although are very comprehensive, do not draw any new conclusion. Most of the figures in the paper are unclear.

This paper presents a concrete testbed for power CPS and this testbed is used to evaluate two attacks (Dos and MitM) against power CPS. The authors thoroughly tested many aspects of impacts to demonstrate the damage caused by the attacks. However, the used techniques and methods are not novel and the authors do not compare their work with other researches. Moreover, the authors detail their experiments by providing a large number of experimental data, but for many of them, I do not understand the meanings. For instance, Figure 20 and Figure 21 depict some detection result, but I cannot get the messages the figures want to deliver. Do these figures only show how to use the Snort utility? My recommendation is that the authors should revise the experiment part to make it clearer. It is unnecessary to present too much data for the experiment, only the crucial data that support the key results should be kept.
}
\end{enumerate}



==> Figures/Patrick_UC_Info.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[height=1 in,width=3.4 in]{Figures/UseCase1/Direct_Operate_Close.png}} %scale=0.2 
\caption{Hexadecimal representation of a normal DNP3 direct operate close packet. }
\label{fig:Direct_Operate_Close}
\end{figure}

%In Fig.~\ref{fig:Direct_Operate_Close} - also this should be in the other part, when we explain the packet structure and show the table. 
%In Fig.~\ref{fig:Generic_DNP3_PAcket_Structure}, the normal hexadecimal representation of a binary direct operate DNP3 packet indicated by the 05 function code. This packet is indexed to close breaker seventh DNP3 point (one of the breakers) in the San Juan substation. This is indicated b the index 07 00, along with the 41 control code used to close the breaker.

\begin{figure}[htbp]
\centerline{\includegraphics[height=1 in,width=3.4 in]{Figures/UseCase1/Direct_Operate_Open.png}} %scale=0.2 
\caption{Hexadecimal representation of a modified DNP3 direct operate open packet. }
\label{fig:Direct_Operate_Open}
\end{figure}

The MiTM ARP cache poisoning reroutes the packets between the outstation and the master, where the binary direct operate is inverted. Meaning that a close command will become a trip or vice-versa. This is shown by Fig.~\ref{fig:Direct_Operate_Open}, an open command being forced to a close command, as shown by Fig.~\ref{fig:Direct_Operate_Open}. Notice that the header information, the function code, and the index remain the unchanged. Only the control code is changed from close (41) to open (81) command. Corresponding the CRC for the DNP3 data is recalculated. It is also important to note the TCP layer checksum is recalculated since the TCP payload is changed. If either the DNP3 CRC or TCP checksum is not updated the outstation will not accept the modified packet.  

\begin{figure}[htbp]
\centerline{\includegraphics[height=1 in,width=3.4 in]{Figures/UseCase1/Direct_Operate_Close_Response.png}} %scale=0.2 
\caption{Hexadecimal representation of a normal DNP3 response packet from outstation that receives a direct operate close packet.}
\label{fig:Direct_Operate_Close_Responce}
\end{figure}

\begin{figure}[htbp]
\centerline{\includegraphics[height=1 in,width=3.4 in]{Figures/UseCase1/Direct_Operate_Open_Response.png}} %scale=0.2 
\caption{Hexadecimal representation of a modified DNP3 response packet from outstation that receives a direct operate close packet.}
\label{fig:Direct_Operate_Close_Responce}
\end{figure}

In order for MiTM to remain undetected by the master, the DNP3 response packet from the outstation is modified to correspond with the original command send. In other words, when the master sends a close command, it is expecting a respond packet stating that the breaker has been closed. 
